Dense Intrinsic Appearance Flow for Human Pose Transfer

We present a novel approach for the task of human pose transfer, which aims at synthesizing a new image of a person from an input image of that person and a target pose. We address the issues of limited correspondences identified between keypoints only and invisible pixels due to self-occlusion. Unlike existing methods, we propose to estimate dense and intrinsic 3D appearance flow to better guide the transfer of pixels between poses. In particular, we wish to generate the 3D flow from just the reference and target poses. Training a network for this purpose is non-trivial, especially when the annotations for 3D appearance flow are scarce by nature. We address this problem through a flow synthesis stage. This is achieved by fitting a 3D model to the given pose pair and project them back to the 2D plane to compute the dense appearance flow for training. The synthesized ground-truths are then used to train a feedforward network for efficient mapping from the input and target skeleton poses to the 3D appearance flow. With the appearance flow, we perform feature warping on the input image and generate a photorealistic image of the target pose. Extensive results on DeepFashion and Market-1501 datasets demonstrate the effectiveness of our approach over existing methods. Our code is available at http://mmlab.ie.cuhk.edu.hk/projects/pose-transfer

==> sections/method_no_segmentation.tex <==
% !TEX root = ../submission_1637.tex

%------------------------------------------------------------------------
\section{Methodology}
\label{sec:method}
%------------------------------------------------------------------------
% Outlines
We first describe the problem setup and notations in Sec~\ref{sec:notation}. Sec.~\ref{sec:framework} gives an overview of our framework (see Fig.~\ref{fig:framework}). Then we introduce the key component of our method, \ie, the flow regression module, in Sec.~\ref{sec:flow_module}, and show how it contributes to pose transfer in Sec.~\ref{sec:feature_warping} and Sec.~\ref{sec:pixel_warping}. Finally, we introduce our loss functions.
%------------------------------------------------------------------------
\subsection{Problem Formulation and Notations}
\label{sec:notation}
%------------------------------------------------------------------------
% Problem setting
Given a reference person image $x$ and a target pose $p$, our goal is to generate a photorealistic person image $\hat{x}$, which retains the identity and clothing appearance of $x$, and has body pose similar to $p$. To achieve arbitrary pose transfer, the pose representation should be both comprehensive and flexible. We use a set of 18 human keypoints extracted by a pose estimator~\cite{cao2017realtime}, following the setting in ~\cite{ma2017pose, siarohin2018deformable}. Specifically, we encode keypoints as a 18-channel binary heatmap, where each channel is filled with 1 within a radius of 8 pixels around the corresponding keypoint and 0 elsewhere. In training, we use the image pair $(x_1, x_2)$ with corresponding poses $(p_1, p_2)$ as the training sample. The model takes $(x_1, p_1, p_2)$ as inputs and tries to generate $\hat{x}_2$ that minimizes an error term between $\hat{x}_2$ and $x_2$.

% Notation of flow
The proposed dense intrinsic appearance flow consist of two components, namely a flow map $F_{(x_1,x_2)}$ and a visibility map $V_{(x_1,x_2)}$, that jointly represent the pixel-wise correspondence between a pair of person images $(x_1,x_2)$. We omit the subscript and write them as $F$ and $V$ for simplicity in the following text. $F$ and $V$ have the same spatial dimensions as $x_2$. Assume that $u_i'$ and $u_i$ are the 2D projection coordinates of the same 3D human body point $h_i$ in $x_1$ and $x_2$ respectively, $F$ and $V$ are defined as:
\begin{equation}\label{eq_flow}
\begin{aligned}
f_i=&F(u_i)=u_i'-u_i, \\
v_i=&V(u_i)=visibility(h_i,x_1),
\end{aligned}
\end{equation}
where $visibility(a_i,x_1)$ is a discrete status function that indicates whether $h_i$ is visible or invisible (self-occluded or off-the-image) in $x_1$.
%------------------------------------------------------------------------
\subsection{Framework}
\label{sec:framework}
%------------------------------------------------------------------------
\begin{figure*}[t]
	\centering
	\includegraphics[width=\linewidth]{framework}
	\vskip -0.25cm
	\caption{Overview of our framework. The input to our method is a triplet $(x_1,p_1,p_2)$, where $x_1$ is a reference image with pose $p_1$. The output is an image $\hat{x}$ that retains the same identity of $x_1$ but in a target pose $p_2$. }
	\label{fig:framework}
	\vskip -0.25cm
\end{figure*}

Our human pose transfer framework is illustrated in Fig.~\ref{fig:framework}. At test time, given the input triplet $(x_1,p_1,p_2)$, the flow regression module first predicts the intrinsic appearance flow $F$ and $V$ as defined in Eqn.~\eqref{eq_flow}. 
%
Then we feed $(x_1,p_2,F,V)$ into the image generator. Note that the reference image $x_1$ and target pose $p_2$ is spatially misaligned, therefore it is hard to capture and fuse appearance/pose information by concatenating $x_1$ and $p_2$ to feed into a unique convolution network, as in~\cite{ma2017pose}. This is because the convolution unit with limited perceptual field is not able to jointly handle signals with large spatial displacement, especially at low-level layers. 

Inspired by~\cite{siarohin2018deformable,zhao2017multi}, our generator adopt a dual-path U-Net architecture. Specifically, two independent convolution encoder networks, denoted as $G_{ea}$ and $G_{ep}$ \cavan{include these notations in the framework figure}, will encode $x_1$ and $p_2$ into hierarchical feature pyramids $\{c_a^k\}$, $\{c_p^k\}$, respectively. 
%
To handle the spatial misalignment between appearance and pose features, we design a flow-guided feature warping module, which warps the appearance feature maps $c_a^k$ according to the flow map $F$ to spatially match the target pose. Meanwhile, the change of visibility of human body parts during pose transfer is also implicitly taken into account by involving visibility map $V$ into the warping operation. 
%
Feature warping is applied at each level in the appearance feature pyramid:
\begin{equation}\label{eq_feat_warp}
\begin{aligned}
c_{aw}^k=W_F(c_a^k, F, V),
\end{aligned}
\end{equation}
where $W_F$ denotes the warping operation, which will be described in detail in Sec.~\ref{sec:feature_warping}. And $\{c^k_{aw}\}$ is the warped appearance feature pyramid. Then we concatenate $\{c_{aw}^k\}$ and $\{c_p^k\}$ at each level, and feed them into the image decoder $G_d$ \cavan{include the notation in the framework figure} through skip connections to generate $\widetilde{x}_2$ with target pose. Finally, we enhance $\widetilde{x}_2$ by a pixel warping module (Sec.~\ref{sec:pixel_warping}) and obtain the finial output image $\hat{x}_2$.

To implement adversarial learning, we adopt a discriminator network that takes the concatenation of tensors $(x_1,p_2,x^*_2)$ as input, where $x^*_2$ is whether the real target image $x_2$ or the generated image $\hat{x}_2$. The output of the discriminator indicates the probability that the input is classified as real sample. Specifically, we adopt the PatchGAN~\cite{pix2pix2016}, which is a convolutional classifier penalizing patch-level structures in images.
%------------------------------------------------------------------------
\subsection{Flow Regression Module}
\label{sec:flow_module}
%------------------------------------------------------------------------
\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{flow_module_no_segmentation}
	\vskip -0.25cm
	\caption{The flow regression module adopts a U-Net architecture that predict the intrinsic appearance flow from a pair of poses. The model is jointly trained using two loss functions, namely an end-point-error loss on the flow map, and a cross-entropy loss on the visibility map.}
	\label{fig:flow_module}
	\vskip -0.25cm
\end{figure}
%------------------------------------------------------------------------
\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{flow_visualization}
	\caption{An illustration of the intrinsic appearance flow in our synthetic dataset (middle) and the predicted result of our flow regression module (right). Note that for the example in the third line, the leg part of the flow map and visibility map is incorrect due to the inaccurate fitting of 3D human model. This has been corrected in the flow regression module prediction.}
	\label{fig:flow_dataset}
\end{figure}
%------------------------------------------------------------------------
Our flow regression module, depicted in Fig.~\ref{fig:flow_module}, is a feedforward CNN that predicts intrinsic appearance flow $F$ and $V$ from the input triplet $(x_1,p_1,p_2)$. The functionality of this module is motivated by the successful applications of CNN in optical flow prediction~\cite{dosovitskiy2015flownet,ilg2017flownet}. However, training such a model requires ground-truth flow data of human motions, which is difficult to obtain. We solve this problem by leveraging 3D human model to generate a synthetic flow dataset. In this section, we first describe the approach we generate the flow dataset, then we will introduce the network architecture and training procedure of our flow regression module.
% synthetic flow dataset

\noindent
\textbf{Synthetic Flow Dataset}. Our approach to synthesize flow data is illustrated in Fig.~\ref{fig:flow_dataset}. We first sample person image pairs with the same identity from a 2D image dataset (in practice, we use the same dataset~\cite{liu2016deepfashion} that we use in pose transfer experiments), denoted as $(x_a,x_b)$\yining{or just $(x_1, x_2)$ if it's not confusing with the notations in Sec.\ref{sec:notation}}. We fit a 3D human model~\cite{loper2015smpl} to both images in the pair, using the state-of-the-art method~\cite{kanazawaHMR18}. The 3D model represents the human body surface with a 3D mesh that consists of 6,890 vertices and 13,766 faces, which can be projected back to the 2D image space using a renderer~\cite{loper2014opendr}. Then for each pixel $u_j$ locating on the human body in $x_b$, we can get the exact mesh face it belongs to and compute its corresponding coordinates $u_j'$ in $x_a$ using barycentric transformation. Thus we can obtain the flow vector as $f_j=u_j'-u_j$. The renderer also provides the visibility status of each faces during projection, from which we can easily compute the visibility map $V$. We also obtain two by-products from each sample, namely a 20-keypoint 2D pose directly output by~\cite{kanazawaHMR18}. This 2D pose can be further converted into the format of 18-channel pose representation used in our main task, denoted as $\widetilde{p}$.

\noindent
\textbf{Network Architecture and Training}. Our flow regression module adopts a U-Net architecture which takes a pair of concatenated pose heatmaps as input and simultaneously generates the flow map and visibility map. We find that this simple network architecture works surprisingly well. We train the flow regression module with two loss functions, namely a end-point-error (EPE) loss on the flow map, and a cross entropy loss on the visibility map.
%
We notice that the inaccuracy in 3D model fitting will cause misalignment between synthesized flow map $\{F,V\}$ and the groundtruth pose $(p_a,p_b)$, which will affect the training of the flow regression module.\yining{will show a sample in~\ref{fig:flow_dataset}} To mitigate the problem, we use $(\widetilde{p}_a, \widetilde{p}_b)$ in training, which is coincident with $\{F,V\}$. Since there is no significant domain gap between $\widetilde{p}$ and $p$, the trained model generalizes well when directly using $p$ as input in testing.
%
And the flow regression module is not jointly trained with the rest of our framework. We pretrain the model separately and fix its parameters when it serves as a module in the pose transfer framework.
%------------------------------------------------------------------------
\subsection{Flow-Guided Feature Warping}
\label{sec:feature_warping}
%------------------------------------------------------------------------
\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{feature_warping_module}
	\vskip -0.25cm
	\caption{Feature warping module.}
	\label{fig:feature_warping_module}
	\vskip -0.25cm
\end{figure}
%------------------------------------------------------------------------
We use a flow-guided feature warping module at each level of the generator to handle the issue of body deformation and the change in visibility. Its architecture is illustrated in Fig.~\ref{fig:feature_warping_module}. 
%
The input includes the appearance feature $c_a^k$ as well as the flow and visibility maps $(F_k,V_k)$, which have been resized to match $c_a^k$. 
%
We first warp the input feature $c_a^k$ towards the target pose using a spatial transformer layer~\cite{jaderberg2015spatial} guided by the flow map $F_k$. The raw warped feature is fed into a spatial gating layer, which divides the feature map into mutually exclusive parts according to the visibility map $V_k$. This is to encode the information of the change of visibility into the feature map. Here we do not operate a hard gating that simply filters off the invisible part, because the feature at invisible region may still contains useful information, like clothing style or body shape. Then the feature map is passed through two convolution layers with residual path to get the final warped feature $c_{aw}^k$. Our feature warping module is differentiable, which allows the gradients to back-propagates from the image decoder $G_d$ to the appearance encoder $G_{ea}$ during training.
%------------------------------------------------------------------------
\subsection{Pixel Warping}
\label{sec:pixel_warping}
%------------------------------------------------------------------------
\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{pixel_warping}
	\vskip -0.25cm
	\caption{Visualization of pixel warping. In each row we show the warped reference image $x_w$,blending weight map $z$, generator output $\widetilde{x}_2$, final result $\hat{x}_2$ and the target image $x_2$.}
	\label{fig:pixel_warping}
	\vskip -0.25cm
\end{figure}
%------------------------------------------------------------------------
Despite the amazing performance of the convolutional image generator in~\cite{karras2018progressive,wang2017high}, it suffers from synthesizing incorrect or degenerated details in pose transfer. One reason is that the convolution layers extract high-level appearance feature from the input image $x_1$ and decode it back to RGB space in the generated image $\widetilde{x}_2$. This process may lose the information of intricate or rare patterns in $x_1$. 

To address this problem, we further exploit the proposed flow representation to directly warp RGB pixels of the reference image $x_1$ and blend them into the generated image. 
%
Specifically, we warp $x_1$ according to the full resolution flow map $F$, and get the a warped image $x_w$ that matches the target pose. $x_w$ is usually distorted because of the loose generated flow and self-occlusion of the human body. 
%
Nevertheless, we can pick out local patterns with fairly good quality from $x_w$, which can be used to enhance $\widetilde{x}_2$. To this end, we add a U-Net into our framework, which takes $x_w$, $\widetilde{x}_2$, $F$ and $V$ as inputs and outputs a one-channel soft weight map $z$ with the same resolution of $x_w$ and $x_2$. The pixel value of $z$ is normalized to a range of $(0,1)$ with sigmoid function. Then the final output $x^*_2$ is computed as a weighted sum of $x_w$ and $\widetilde{x}_2$ as:
\begin{equation}\label{eq_blend}
\begin{aligned}
\hat{x}_2 = z \cdot x_w + (1-z) \cdot \widetilde{x}_2.
\end{aligned}
\end{equation}

Fig.~\ref{fig:pixel_warping} shows the effect of pixel warping. The model is able to focus on the regions with complex high-frequency pattern that can not be well generated by the generator. These patterns will be directly copy from the warped reference image to enhance final result.

%------------------------------------------------------------------------
\subsection{Loss Functions}
\label{sec:loss_functions}
%------------------------------------------------------------------------
The goal of our model is to achieve arbitrary and accuracy human pose transfer, and generate photorealistic human image. This task is challenging due to the large non-rigid deformation during pose transfer and complex appearance details in human images. Previous works on conditional image generation~\cite{pix2pix2016,wang2017high} and human pose transfer~\cite{ma2017pose,siarohin2018deformable,neverova2018dense} utilize multiple loss functions to jointly control the training process. In this work we use a combination of three loss functions in the training phase, namely an adversarial loss $\mathcal{L}_{adv}$, an L1 reconstruction loss $\mathcal{L}_{L1}$, and a perceptual loss $\mathcal{L}_{perceptual}$. We next introduce these items in detail.

\noindent
\textbf{Adversarial Loss.} We adopt a vanilla GAN loss in the conditional setting in our task, which is defined as:
\begin{equation}\label{eq_loss_gan}
\begin{aligned}
\mathcal{L}_{adv}(G,D) = &E_{x_1,x_2}[logD(x_2|x_1,p_2)] \\+ &E_{x_1,x_2}[log(1-D(G(x_1,p_2)|x_1,p_2))].
\end{aligned}
\end{equation}

\noindent
\textbf{L1 Loss.} Previous work~\cite{pix2pix2016} shows L1 loss can stabilize the training process when a target groundtruth is available. Therefore we also adopt a L1 constraint between the generated image and the target image as:
\begin{equation}\label{eq_loss_l1}
\begin{aligned}
\mathcal{L}_{L1}(G) = ||\hat{x}_2 - x_2||_1.
\end{aligned}
\end{equation}

\noindent
\textbf{Perceptual Loss.}~\cite{johnson2016perceptual} shows that penalizing L2-distance between feature maps extracted from two images by a pretrained CNN could enforce structure similarity. We adopt a VGG19 network~\cite{simonyan2014very} pretrained on ImageNet~\cite{russakovsky2015imagenet} as the feature extractor, and use multi-level feature maps $\phi_j$ to compute perceptual loss as:
\begin{equation}\label{eq_loss_perceptual}
\begin{aligned}
\mathcal{L}_{perceptual}(G) = \sum_{j=1}^{N}||\phi_j(\hat{x}_2)-\phi_j(x_2)||^2_2.
\end{aligned}
\end{equation}
Our final generator loss function is a weighted sum of above terms, as follows.
\begin{equation}\label{eq_loss_total}
\begin{aligned}
\mathcal{L}(G) = \lambda_1\mathcal{L}_{adv}+\lambda_2\mathcal{L}_{L1}+\lambda_3\mathcal{L}_{perceptual}.
\end{aligned}
\end{equation}




==> sections/method_old.tex <==
%------------------------------------------------------------------------
\section{Method}
\label{sec:method}
%------------------------------------------------------------------------
%------------------------------------------------------------------------
\subsection{Flow Generation Module}
\label{sec:flow_module}
%------------------------------------------------------------------------
Our flow generation module consists of two cascaded networks, namely a segmentation generator and a flow generator, both have a U-Net architecture. The segmentation generator takes a pose representation $p$ (a 18-channel heatmap of human joint points) as input, and outputs a 7-class segmentation map $s$. The input of the flow generator is pose representations and segmentation maps from a pair of images $(x1, x2)$. These input tensors are concatenated along the channel dimension before fed into the flow generator. And the flow generator will output a predicted flow map $f$ from $x_2$ to $x_1$, and a visibility map $v$ which indicates whether a pixel in $x_2$ is corresponding to a visible part in $x_1$.

The segmentation generator and flow generator are trained separately. The training data, including joint poses, segmentation maps, flow maps and visibility maps, denoted as $(p', s', f', v')$, are all obtained from SMPL models fitted to real images. Note that here we use joint locations from SMPL as pose representation, instead of joint locations detected by LIP\misscite which are used in pose transfer model (\ref{sec:pose_transfer}). The reason is to keep the consistency of pose, segmentation and flow during training the flow generation module, and mitigate the influence of SMPL fitting errors.

\begin{figure}[h]
	\centering
	\includegraphics[width=\linewidth]{seg_train}
	\vskip -0.25cm
	\caption{Training of segmentation generator.}
	\label{fig:seg_train}
	\vskip -0.25cm
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=\linewidth]{flow_train}
	\vskip -0.25cm
	\caption{Training of flow generator.}
	\label{fig:flow_train}
	\vskip -0.25cm
\end{figure}

\begin{figure}[h]
	\centering
	\includegraphics[width=\linewidth]{flow_test}
	\vskip -0.25cm
	\caption{Inferring process of flow generation module.}
	\label{fig:flow_test}
	\vskip -0.25cm
\end{figure}

%------------------------------------------------------------------------
\subsection{Flowed Guided Pose Transfer}
\label{sec:pose_transfer}
%------------------------------------------------------------------------
\begin{figure}[h]
	\centering
	\includegraphics[width=\linewidth]{pipeline_unet}
	\vskip -0.25cm
	\caption{A simple pose transfer pipeline using a single U-Net\misscite as image generator. }
	\label{fig:pipepine_unet}
	\vskip -0.25cm
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=\linewidth]{pipeline_2stage}
	\vskip -0.25cm
	\caption{A 2-stage pipeline that contains a image generator and a image refiner.}
	\label{fig:pipeline_2stage}
	\vskip -0.25cm
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=\linewidth]{pipeline_fw}
	\vskip -0.25cm
	\caption{The appearance information is extracted into multi-level features by a encoder network. Then the appearance features are warped towards target pose guided by predicted flow. The network architecture is similar to Deformable-GAN\misscite.}
	\label{fig:pipeline_fw}
	\vskip -0.25cm
\end{figure}

%------------------------------------------------------------------------
\subsection{Implementation Details}
\label{sec:implementation}
%------------------------------------------------------------------------
